On Bias and Fairness in NLP: Investigating the Impact of Bias and Debiasing in Language Models on the Fairness of Toxicity Detection

Language models are the new state-of-the-art natural language processing (NLP) models and they are being increasingly used in many NLP tasks. Even though there is evidence that language models are biased, the impact of that bias on the fairness of downstream NLP tasks is still understudied. Furthermore, despite that numerous debiasing methods have been proposed in the literature, the impact of bias removal methods on the fairness of NLP tasks is also understudied. In this work, we investigate three different sources of bias in NLP models, i.e. representation bias, selection bias and overamplification bias, and examine how they impact the fairness of the downstream task of toxicity detection. Moreover, we investigate the impact of removing these biases using different bias removal techniques on the fairness of toxicity detection. Results show strong evidence that downstream sources of bias, especially overamplification bias, are the most impactful types of bias on the fairness of the task of toxicity detection. We also found strong evidence that removing overamplification bias by fine-tuning the language models on a dataset with balanced contextual representations and ratios of positive examples between different identity groups can improve the fairness of the task of toxicity detection. Finally, we build on our findings and introduce a list of guidelines to ensure the fairness of the task of toxicity detection.

==> random.tex <==
\section{Sentiment analysis task}
\begin{table*}[]
\begin{tabular}{|lrlll|}
\hline
\multicolumn{1}{|l|}{Model}                                           & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Albert}                                          & \multicolumn{1}{r|}{0.865} & \multicolumn{1}{l|}{0.01}     & \multicolumn{1}{l|}{0.008}    & 0.002    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                    & \multicolumn{1}{r|}{0.855} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.02$}     & 0.002    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                  & \multicolumn{1}{r|}{0.435} & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{red}$\uparrow0.008$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                     & \multicolumn{1}{r|}{0.869} & \multicolumn{1}{l|}{\color{red}$\uparrow0.019$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{teal}$\downarrow0$        \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-downstream-counterfactual} & \multicolumn{1}{r|}{0.864} & \multicolumn{1}{l|}{0.01}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{5}{|l|}{}                                                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{Model}                                           & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{BERT}                                            & \multicolumn{1}{r|}{0.86}  & \multicolumn{1}{l|}{0.029}    & \multicolumn{1}{l|}{0.008}    & 0.006    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                    & \multicolumn{1}{r|}{0.862} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.012$}    & \color{teal}$\downarrow0$        \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                  & \multicolumn{1}{r|}{0.42}  & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{teal}$\downarrow0.005$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                     & \multicolumn{1}{r|}{0.852} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.019$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-downstream-counterfactual} & \multicolumn{1}{r|}{0.859} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{5}{|l|}{}                                                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{Model}                                           & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Roberta}                                         & \multicolumn{1}{r|}{0.878} & \multicolumn{1}{l|}{0.01}     & \multicolumn{1}{l|}{0.008}    & 0.002    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                    & \multicolumn{1}{r|}{0.897} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                  & \multicolumn{1}{r|}{0.482} & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{red}$\uparrow0.007$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                     & \multicolumn{1}{r|}{0.878} & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.02$}     & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-downstream-counterfactual} & \multicolumn{1}{r|}{0.89}  & \multicolumn{1}{l|}{\color{red}$\uparrow0.029$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.012$}    & \color{teal}$\downarrow0.001$    \\ \hline
\end{tabular}
\end{table*}


\begin{table}[h]
    \renewcommand{\arraystretch}{1}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{|lllll|}
\hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : gender}}                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Albert}                                                                                                           & \multicolumn{1}{l|}{0.847} & \multicolumn{1}{l|}{0.006}    & \multicolumn{1}{l|}{0.039}    & 0.004    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                                                                                     & \multicolumn{1}{l|}{0.840} & \multicolumn{1}{l|}{0.006}    & \multicolumn{1}{l|}{\color{teal} $\downarrow 0.032$}    & 0.004   \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                                                                                   & \multicolumn{1}{l|}{0.524}      & \multicolumn{1}{l|}{\color{teal}$\downarrow 0$}        & \multicolumn{1}{l|}{\color{teal} $\downarrow 0.008$}    & \color{red} $\uparrow 0.011$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.848}      & \multicolumn{1}{l|}{\color{teal}$\downarrow 0.001$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.01$}     & 0.004    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.816}      & \multicolumn{1}{l|}{\color{teal} $\downarrow0.005$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.003$}    & \color{red}$\uparrow0.005$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.803}      & \multicolumn{1}{l|}{\color{teal} $\downarrow0.005$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.006$}    & \color{red} $\uparrow0.008$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-gender-\\           downstream-all-data-debias\end{tabular}}     & \multicolumn{1}{l|}{0.792}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.005$}    & \color{red} $\uparrow0.008$    \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : race}}                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Albert}                                                                                                           & \multicolumn{1}{l|}{0.847} & \multicolumn{1}{l|}{0.008}    & \multicolumn{1}{l|}{0.002}    & 0.019    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-race}                                                                                       & \multicolumn{1}{l|}{0.838}      & \multicolumn{1}{l|}{\color{teal} $\downarrow0.003$}    & \multicolumn{1}{l|}{\color{red} $\uparrow 0.003$}    & \color{teal} $\downarrow0.013$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-race}                                                                                     & \multicolumn{1}{l|}{0.421}      & \multicolumn{1}{l|}{\color{teal} $\downarrow 0$}        & \multicolumn{1}{l|}{\color{red} $\uparrow0.004$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.848}      & \multicolumn{1}{l|}{\color{teal} $\downarrow0.003$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.001$}    & \color{teal} $\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.816}      & \multicolumn{1}{l|}{\color{red} $\uparrow0.022$}    & \multicolumn{1}{l|}{\color{red} $\uparrow0.026$}    & \color{teal} $\downarrow0.008$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.803}      & \multicolumn{1}{l|}{\color{red}$\uparrow0.004$}    & \multicolumn{1}{l|}{0.002}    & \color{teal} $\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-race-\\           downstream-all-data-debias\end{tabular}}       & \multicolumn{1}{l|}{0.817}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{red} $\uparrow0.017$}    & \color{teal} $\downarrow0.001$    \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : religion}}                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Albert}                                                                                                           & \multicolumn{1}{l|}{0.847} & \multicolumn{1}{l|}{0.01}     & \multicolumn{1}{l|}{0.109}    & 0.02     \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-religion}                                                                                   & \multicolumn{1}{l|}{0.837}      & \multicolumn{1}{l|}{\color{red} $\uparrow0.019$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.094$}    & \color{teal}$\downarrow0.016$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-religion}                                                                                 & \multicolumn{1}{l|}{0.507}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0$}        & \color{teal} $\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.848}      & \multicolumn{1}{l|}{\color{teal} $\downarrow0.002$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.011$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.816}      & \multicolumn{1}{l|}{\color{red}$\uparrow0.03$}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.058$}    & \color{teal}$\downarrow0$        \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.803}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow 0.002$}    & \color{teal} $\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-religion-\\             downstream-all-data-debias\end{tabular}} & \multicolumn{1}{l|}{0.811}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal} $\downarrow0.013$}    & \color{teal}$\downarrow0.003$    \\ \hline
\end{tabular}}
\caption{Performance and fairness scores of the Albert model on the balanced toxicity fairness datasets.}
\label{tab:extrinsic_bias_scores_jigsaw_dataset_albert}
\end{table}
\begin{table}[h]
    \renewcommand{\arraystretch}{1}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{|lllll|}
\hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : gender}}                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}  & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Bert}                                                                                                             & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.09}     & \multicolumn{1}{l|}{0.036}    & 0.01     \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                                                                                     & \multicolumn{1}{l|}{0.841}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.011$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.049$}    & \color{teal}$\downarrow0.006$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                                                                                   & \multicolumn{1}{l|}{0.478}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal} $\downarrow0.001$}    & \color{teal}$\downarrow0.004$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.837}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.817}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.007$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.006$}    & \color{teal}$\downarrow0.006$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.810}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \color{teal}$\downarrow0.005$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-gender-\\           downstream-all-data-debias\end{tabular}}     & \multicolumn{1}{l|}{0.791}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : race}}                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}  & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Bert}                                                                                                             & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.016}    & \multicolumn{1}{l|}{0.002}    & 0.026    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-race}                                                                                       & \multicolumn{1}{l|}{0.829}     & \multicolumn{1}{l|}{\color{red}$\uparrow.021$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.005$}    & \color{teal}$\downarrow0.024$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-race}                                                                                     & \multicolumn{1}{l|}{0.504}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.837}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.009$}    & \multicolumn{1}{l|}{\color{red}$\uparrow0.019$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.817}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.01$}     & \multicolumn{1}{l|}{\color{red}$\uparrow.018$}    & \color{teal}$\downarrow0.008$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.810}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.002$}    & \multicolumn{1}{l|}{0.002}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-race-\\           downstream-all-data-debias\end{tabular}}       & \multicolumn{1}{l|}{0.815}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \multicolumn{1}{l|}{0.002}    & \color{teal}$\downarrow0$        \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : religion}}                                                                                                                                                                                 \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}  & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Bert}                                                                                                             & \multicolumn{1}{l|}{0.83} & \multicolumn{1}{l|}{0.008}    & \multicolumn{1}{l|}{0.063}    & 0.012    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-religion}                                                                                   & \multicolumn{1}{l|}{0.833}     & \multicolumn{1}{l|}{\color{red}$\uparrow.015$}    & \multicolumn{1}{l|}{\color{red}$\uparrow.084$}    & \color{red}$\uparrow.017$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-religion}                                                                                 & \multicolumn{1}{l|}{0.447}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{red}$\uparrow.03$     \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.837}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.002$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.011$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.817}     & \multicolumn{1}{l|}{\color{red}$\uparrow.02$}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0.049$}    & \color{teal}$\downarrow0.006$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.810}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-religion-\\             downstream-all-data-debias\end{tabular}} & \multicolumn{1}{l|}{0.820}     & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \color{teal}$\downarrow0.003$    \\ \hline
\end{tabular}}
\caption{Performance and fairness scores of the BERT model on the balanced toxicity fairness datasets.}
\label{tab:extrinsic_bias_scores_jigsaw_dataset_bert}
\end{table}
\begin{table}[h]
    \renewcommand{\arraystretch}{1}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{|lllll|}
\hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : gender}}                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Roberta}                                                                                                          & \multicolumn{1}{l|}{0.851} & \multicolumn{1}{l|}{0.005}    & \multicolumn{1}{l|}{0.032}    & 0.011    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-gender}                                                                                     & \multicolumn{1}{l|}{0.856}      & \multicolumn{1}{l|}{\color{red}$\uparrow0.006$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.022$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-gender}                                                                                   & \multicolumn{1}{l|}{0.520}      & \multicolumn{1}{l|}{\color{red}$\uparrow.015$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.019$}    & \color{teal}$\downarrow0.004$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.873}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.009$}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.842}      & \multicolumn{1}{l|}{\color{red}$\uparrow.006$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.825}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0.005$}    & \color{teal}$\downarrow0.007$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-gender-\\           downstream-all-data-debias\end{tabular}}     & \multicolumn{1}{l|}{0.837}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \color{teal}$\downarrow0.004$    \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : race}}                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Roberta}                                                                                                          & \multicolumn{1}{l|}{0.851} & \multicolumn{1}{l|}{0.003}    & \multicolumn{1}{l|}{0.011}    & 0.021    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-race}                                                                                       & \multicolumn{1}{l|}{0.854}      & \multicolumn{1}{l|}{\color{red}$\uparrow.017$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.009$}    & 0.021    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-race}                                                                                     & \multicolumn{1}{l|}{0.561}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{teal}$\downarrow0.005$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.873}      & \multicolumn{1}{l|}{\color{red}$\uparrow.018$}    & \multicolumn{1}{l|}{\color{red}$\uparrow.038$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.842}      & \multicolumn{1}{l|}{\color{red}$\uparrow.014$}    & \multicolumn{1}{l|}{0.011}    & \color{teal}$\downarrow0.014$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.825}      & \multicolumn{1}{l|}{0.003}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.006$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-race-\\           downstream-all-data-debias\end{tabular}}       & \multicolumn{1}{l|}{0.842}      & \multicolumn{1}{l|}{\color{red}$\uparrow.006$}    & \multicolumn{1}{l|}{\color{red}$\uparrow.014$}    & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{5}{|c|}{\textbf{Sensitive attribute : religion}}                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{Model}                                                                                                            & \multicolumn{1}{l|}{AUC}   & \multicolumn{1}{l|}{FPR\_gap} & \multicolumn{1}{l|}{TPR\_gap} & AUC\_gap \\ \hline
\multicolumn{1}{|l|}{Roberta}                                                                                                          & \multicolumn{1}{l|}{0.851} & \multicolumn{1}{l|}{0.022}    & \multicolumn{1}{l|}{0.16}     & 0.027    \\ \hline
\multicolumn{1}{|l|}{+ upstream-sentDebias-religion}                                                                                   & \multicolumn{1}{l|}{0.843}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.021$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.10$}     & \color{teal}$\downarrow0.003$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-sentDebias-religion}                                                                                 & \multicolumn{1}{l|}{0.523}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \color{teal}$\downarrow0$        \\ \hline
\multicolumn{1}{|l|}{+ downstream-perturbed-data}                                                                                      & \multicolumn{1}{l|}{0.873}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.003$}    & \color{teal}$\downarrow0.002$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-data}                                                                                     & \multicolumn{1}{l|}{0.842}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.019$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.071$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{+ downstream-stratified-perturbed-data}                                                                           & \multicolumn{1}{l|}{0.825}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0.001$}    & \multicolumn{1}{l|}{\color{teal}$\downarrow0.004$}    & \color{teal}$\downarrow0.001$    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}+ upstream-sentDebias-religion-\\             downstream-all-data-debias\end{tabular}} & \multicolumn{1}{l|}{0.834}      & \multicolumn{1}{l|}{\color{teal}$\downarrow0$}        & \multicolumn{1}{l|}{\color{teal}$\downarrow0.006$}    & \color{teal}$\downarrow0.007$    \\ \hline
\end{tabular}}
\caption{Performance and fairness scores of the RoBERTa model on the balanced toxicity fairness datasets.}
\label{tab:extrinsic_bias_scores_jigsaw_dataset_roberta}
\end{table}

\begin{table*}[ht]
    \centering
    \renewcommand{\arraystretch}{1.05}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{lllrrrr}
    \hline
         Attribute & Model & Dataset & AUC & FPR\_gap & TPR\_gap & AUC\_gap  \\
    \hline
         \multirow{6}{*}{Gender} &
         \multirow{2}{*}{ALBERT} &
         Original & 0.911 & 0.001 & 0.081 & 0.025 \\
    & &  Balanced & 0.847 & \color{red}$\uparrow0.006$    &  \color{teal}$\downarrow0.038$   &  \color{teal}$\downarrow0.003$ \\
    \cline{2-7}
    &     \multirow{2}{*}{BERT}
      &  Original & 0.902 & 0.002 &  0.111 & 0.026 \\
    & &  Balanced & 0.830 & \color{red}$\uparrow0.008$    &  \color{teal}$\downarrow0.036$   &  \color{teal}$\downarrow0.009$ \\
    \cline{2-7}
    &     \multirow{2}{*}{RoBERTa}
      &  Original & 0.908 & 0.007 &  0.084 & 0.017 \\
    & &  Balanced & 0.851 & \color{teal}$\downarrow0.004$    &  \color{teal}$\downarrow0.031$   &  \color{teal}$\downarrow0.011$ \\
    \hline
         \multirow{6}{*}{Race} &
         \multirow{2}{*}{ALBERT} &
         Original & 0.911 &  0.007 &   0.044 &  0.003\\
    & &  Balanced & 0.847 &  \color{red}$\uparrow0.008$   &   \color{teal}$\downarrow0.0016$   &  \color{red}$\uparrow0.018$ \\
    \cline{2-7}
    &     \multirow{2}{*}{BERT}
      &  Original &  0.902 &  0.008 &   0.017 &  0.048 \\
    & &  Balanced & 0.830 &  \color{red}$\uparrow0.015$   &   \color{teal}$\downarrow0.002$   &  \color{teal}$\downarrow0.025$ \\
    \cline{2-7}
    &     \multirow{2}{*}{RoBERTa}
      &  Original & 0.908 &  0.014 &   0.127 &  0.028 \\
    & &  Balanced & 0.851 &  \color{teal}$\downarrow0.003$   &   \color{teal}$\downarrow0.011$  &  \color{teal}$\downarrow0.021$ \\
    \hline
         \multirow{6}{*}{Religion} &
         \multirow{2}{*}{ALBERT} &
         Original & 0.911  &  0.019 &  0.060  &   0.042 \\
    & &  Balanced & 0.847 &   \color{teal}$\downarrow0.009$  &   \color{red}$\uparrow0.108$   &  \color{teal}$\downarrow0.020$ \\
    \cline{2-7}
    &     \multirow{2}{*}{BERT}
      &  Original & 0.902  &  0.016 &  0.027  &   0.051 \\
    & &  Balanced & 0.830 &   \color{teal}$\downarrow0.008$  &   \color{red}$\uparrow0.062$   &  \color{teal}$\downarrow0.012$ \\
    \cline{2-7}
    &     \multirow{2}{*}{RoBERTa}
      &  Original & 0.908  &  0.027 &  0.030  &   0.0369 \\
    & &  Balanced & 0.851 &   \color{teal}$\downarrow0.021$  &   \color{red}$\uparrow0.160$   &  \color{teal}$\downarrow0.027$ \\
    \hline
    \end{tabular}
    } % resizebox
    \caption{Toxicity detection performance and fairness scores for the original and the balanced datasets using the examined ALBERT, BERT, and RoBERTa models.}
    \label{tab:extrinsic_bias_scores_perturbed_vs_original_jigsaw_dataset}
\end{table*}
